Quantum-router: Storing and redirecting light at the photon level

We propose a method for spatially re-routing single photons or light in a coherent state with small average photon number by purely electronic means, i.e. without using mechanical devices such as micro-mirror arrays. The method is based on mapping the quantum state of the incoming light onto a spin-wave in an atomic ensemble as is done in quantum memories of light. Then the wavevector of the spin-wave is modified in a controlled way by an applied magnetic field gradient. Finally, by re-applying the same control beam as for storing, the signal pulse is released in a new direction that depends on the deflected wavevector of the spin-wave. We show by numerical simulation that efficiencies can be achieved for arbitrary deflection angles in the plane that are comparable with simple photon storage and re-emission in forward direction, and propose a new method for eliminating the stored momentum as source of decoherence in the quantum memory. In a reasonable parameter regime, the re-routing should be achievable on a time-scale on the order of few to $\sim100$ microseconds, depending on the deflection angle. The shifts in the wavevector that can be achieved using the Zeeman-effect, with otherwise minimal changes to the spin-wave, can also be used to complement existing ac-Stark spin-wave manipulation methods.

==> img/opt_em_w100_c850_d6_th0/params_Absorption.tex <==
$\theta$& 0.00 \\ 
$\tilde{w}_{\mathcal{E},\parallel}$& 100.00 \\ 
$\tilde{w}_{\mathcal{E},\perp}$& 0.20 \\ 
$\tilde{A}_\Omega$& 8.82 \\ 
$\tilde{c}{t}_{0,\Omega}$& -43.97 \\ 
$\tilde{x}_{0,\Omega}$& -5.13 \\ 
$\tilde{y}_{0,\Omega}$& 0.00 \\ 
$\tilde{w}_{\Omega,\parallel}$& 90.91 \\ 
$\tilde{w}_{\Omega,\perp}$& 1.80 \\ 
$\eta_\text{abs}$& 0.71 \\ 


==> img/opt_em_w100_c850_d6_th0/params_Emission.tex <==
$\theta'$& 0.00 \\ 
$\tilde{A}'_\Omega$& 8.87 \\ 
$\tilde{c}\tilde{t}'_{0,\Omega}$& -57.97 \\ 
$\tilde{x}'_{0,\Omega}$& -35.13 \\ 
$\tilde{y}'_{0,\Omega}$& 0.00 \\ 
$\tilde{w}'_{\Omega,\parallel}$& 90.91 \\ 
$\tilde{w}'_{\Omega,\perp}$& 1.80 \\ 
$\eta_\text{em}$& 0.58 \\ 


==> img/opt_em_w100_c850_d6_th0/params_Manipulation.tex <==
manipulation mode& ideal\\ 
$\varphi$& 0.00 \\ 
$\tilde{A}_\Omega$& 25.00 \\ 
$\tilde{c}\tilde{t}_{0,\Omega}$& 0.00 \\ 
$\tilde{x}_{0,\Omega}$& 0.00 \\ 
$\tilde{y}_{0,\Omega}$& 0.00 \\ 
$\tilde{w}_{\Omega,\parallel}$& 80.00 \\ 
$\tilde{w}_{\Omega,\perp}$& 7.00 \\ 
$\theta$& 0.00 \\ 
control shape& rect\\ 
$\tilde{\Delta}$& 100.00 \\ 
$\eta_\text{man}$& 1.00 \\ 


==> img/opt_em_w100_c850_d6_th0/params_System.tex <==
$\tilde{c}$& 850.00 \\ 
$\tilde{g}$& 71.41 \\ 
$\tilde{\Delta}$& 0.00 \\ 

